A Multi-Level Simulation Optimization Approach for Quantile Functions

Quantile is a popular performance measure for a stochastic system to evaluate its variability and risk. To reduce the risk, selecting the actions that minimize the tail quantiles of some loss distributions is typically of interest for decision makers. When the loss distribution is observed via simulations, evaluating and optimizing its quantile functions can be challenging, especially when the simulations are expensive, as it may cost a large number of simulation runs to obtain accurate quantile estimators. In this work, we propose a multi-level metamodel (co-kriging) based algorithm to optimize quantile functions more efficiently. Utilizing non-decreasing properties of quantile functions, we first search on cheaper and informative lower quantiles which are more accurate and easier to optimize. The quantile level iteratively increases to the objective level while the search has a focus on the possible promising regions identified by the previous levels. This enables us to leverage the accurate information from the lower quantiles to find the optimums faster and improve algorithm efficiency.

==> Mutilevel quantile optimization/StdDef.tex <==
\global\long\def\EE{\mathbb{E}}

\global\long\def\PP{\mathbb{P}}

\global\long\def\RR{\mathbb{R}}

\global\long\def\ZZ{\mathbb{Z}}

\global\long\def\NN{\mathbb{N}}

\global\long\def\TT{\mathbb{T}}
\global\long\def\UU{\mathbb{U}}
\global\long\def\VV{\mathbb{V}}
\global\long\def\WW{\mathbb{W}}
\global\long\def\SS{\mathbb{S}}

\global\long\def\FF{\mathbb{F}}
\global\long\def\XX{\mathbb{X}}
\global\long\def\YY{\mathbb{Y}}
\global\long\def\ZZ{\mathbb{Z}}
\global\long\def\AA{\mathbb{A}}

\global\long\def\Ff{\mathcal{F}}
\global\long\def\Hh{\mathcal{H}}
\global\long\def\Vv{\mathcal{V}}
\global\long\def\Cc{\mathcal{C}}
\global\long\def\Ii{\mathcal{I}}

\global\long\def\Ll{\mathcal{L}}
\global\long\def\Pp{\mathcal{P}}
\global\long\def\Oo{\mathcal{O}}
\global\long\def\Mm{\mathcal{M}}

\global\long\def\pP{\mathscr{P}}
\global\long\def\lL{\mathscr{L}}
\global\long\def\bB{\mathscr{B}}
\global\long\def\dD{\mathscr{D}}
\global\long\def\rR{\mathscr{R}}

\global\long\def\RrR{\mathfrak{R}}
\global\long\def\PpP{\mathfrak{P}}
\global\long\def\XxX{\mathfrak{X}}
\global\long\def\YyY{\mathfrak{Y}}
\global\long\def\ZzZ{\mathfrak{Z}}
\global\long\def\ddD{\mathfrak{d}}
\global\long\def\mmM{\mathfrak{m}}
\global\long\def\nnN{\mathfrak{n}}
\global\long\def\TtT{\mathfrak{T}}
\global\long\def\CcC{\mathfrak{C}}
\global\long\def\EeE{\mathfrak{E}}
\global\long\def\AaA{\mathfrak{A}}
\global\long\def\BbB{\mathfrak{B}}

\global\long\def\iiI{\mathfrak{i}}
\global\long\def\jjJ{\mathfrak{j}}
\global\long\def\kkK{\mathfrak{k}}
\global\long\def\llL{\mathfrak{l}}
\global\long\def\mmM{\mathfrak{m}}
\global\long\def\nnN{\mathfrak{n}}

\global\long\def\D{\mathrm{d}}

\global\long\def\E{\mathrm{e}}

\global\long\def\Reals{\RR}
\global\long\def\RealsNN{\RR_{\geq0}}
\global\long\def\RealsP{\RR_{>0}}

\global\long\def\deq{\coloneqq}
\global\long\def\eqd{\eqqcolon}
\global\long\def\dom{\mathop{\mathrm{dom}}}
\global\long\def\argmax{\mathop{\mathrm{arg\,max}}}
\global\long\def\argmin{\mathop{\mathrm{arg\,min}}}
\global\long\def\supp{\mathop{\mathrm{supp}}}

\global\long\def\transp{\top}
\global\long\def\indic{\mathbb{\mathrm{1}}}

\global\long\def\trace{\mathop{\mathrm{Tr}}}
\global\long\def\CVaR{\mathop{\mathrm{CVaR}}}

\global\long\def\DF{\mathrm{D}}
\global\long\def\SD{\text{\ensuremath{\partial}}}

\global\long\def\colplus{\oplus}
\global\long\def\rowplus{\oplus}
\global\long\def\diag{\mathop{\mathrm{diag}}}

\global\long\def\cddot{\mathop{\cdot\cdot}}

\global\long\def\deltaX{\hat{X}}
\global\long\def\deltaY{\hat{Y}}
\global\long\def\deltaZ{\hat{Z}}
\global\long\def\deltaU{\hat{U}}
\global\long\def\deltaB{\hat{B}}
\global\long\def\deltaSigma{\hat{\Sigma}}
\global\long\def\deltaF{\hat{F}}
\global\long\def\deltaPhi{\hat{\Phi}}

\global\long\def\deltaXast{\deltaX^{\ast}}
\global\long\def\deltaYast{\deltaY^{\ast}}
\global\long\def\deltaZast{\deltaZ^{\ast}}
\global\long\def\deltaUast{\deltaU^{\ast}}

\global\long\def\interior{\mathop{\mathrm{int}}}
\global\long\def\sgn{\mathop{\mathrm{sgn}}}
\global\long\def\cvar{\mathbb{ES}}
\global\long\def\var{\mathrm{VaR}}
\global\long\def\as{\text{-a.s.}}

\global\long\def\warrow{\stackrel{\text{w}}{\longrightarrow}}
\global\long\def\wsarrow{\stackrel{\text{w}^{\ast}}{\longrightarrow}}

\global\long\def\cl{\mathop{\mathrm{cl}}}
\global\long\def\diam{\mathop{\mathrm{diam}}}
\global\long\def\ba{\mathrm{ba}}

\global\long\def\rhoMD{\rho^{\mathrm{MD}}}
\global\long\def\rhoMSD{\rho^{\mathrm{MD+}}}
\global\long\def\rhoEpsMSD{\rho_{\epsilon}^{\mathrm{MD+}}}
\global\long\def\rhoEntr{\rho^{\mathrm{Ent}}}


